Generalizable Person Re-identification with Relevance-aware Mixture of Experts

Domain generalizable (DG) person re-identification (ReID) is a challenging problem because we cannot access any unseen target domain data during training. Almost all the existing DG ReID methods follow the same pipeline where they use a hybrid dataset from multiple source domains for training, and then directly apply the trained model to the unseen target domains for testing. These methods often neglect individual source domains' discriminative characteristics and their relevances w.r.t. the unseen target domains, though both of which can be leveraged to help the model's generalization. To handle the above two issues, we propose a novel method called the relevance-aware mixture of experts (RaMoE), using an effective voting-based mixture mechanism to dynamically leverage source domains' diverse characteristics to improve the model's generalization. Specifically, we propose a decorrelation loss to make the source domain networks (experts) keep the diversity and discriminability of individual domains' characteristics. Besides, we design a voting network to adaptively integrate all the experts' features into the more generalizable aggregated features with domain relevance. Considering the target domains' invisibility during training, we propose a novel learning-to-learn algorithm combined with our relation alignment loss to update the voting network. Extensive experiments demonstrate that our proposed RaMoE outperforms the state-of-the-art methods.

==> reference <==
@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})



@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})



@misc{Authors14,
 author = {FirstName LastName},
 title = {The frobnicatable foo filter},
 note = {Face and Gesture  submission ID 324. Supplied as additional material {\tt fg324.pdf}},
 year = 2014
}

@misc{Authors14b,
 author = {FirstName LastName},
 title = {Frobnication tutorial},
 note = {Supplied as additional material {\tt tr.pdf}},
 year = 2014
}

@article{Alpher02,
author = {FirstName Alpher},
title = {Frobnication},
journal = PAMI,
volume = 12, 
number = 1, 
pages = {234--778}, 
year = 2002
}

@article{Alpher03,
author = {FirstName Alpher and  FirstName Fotheringham-Smythe},
title = {Frobnication revisited},
journal = {Journal of Foo},
volume = 13, 
number = 1, 
pages = {234--778}, 
year = 2003
}

@article{Alpher04,
author = {FirstName Alpher and FirstName Fotheringham-Smythe and FirstName Gamow},
title = {Can a machine frobnicate?},
journal = {Journal of Foo},
volume = 14, 
number = 1, 
pages = {234--778}, 
year = 2004
}

@article{sun2019learning,
  title={Learning part-based convolutional features for person re-identification},
  author={Sun, Yifan and Zheng, Liang and Li, Yali and Yang, Yi and Tian, Qi and Wang, Shengjin},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  year={2019},
  publisher={IEEE}
}

@inproceedings{zheng2019joint,
  title={Joint discriminative and generative learning for person re-identification},
  author={Zheng, Zhedong and Yang, Xiaodong and Yu, Zhiding and Zheng, Liang and Yang, Yi and Kautz, Jan},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={2138--2147},
  year={2019}
}

@inproceedings{hou2019interaction,
  title={Interaction-and-aggregation network for person re-identification},
  author={Hou, Ruibing and Ma, Bingpeng and Chang, Hong and Gu, Xinqian and Shan, Shiguang and Chen, Xilin},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={9317--9326},
  year={2019}
}

@inproceedings{chen2019abd,
  title={Abd-net: Attentive but diverse person re-identification},
  author={Chen, Tianlong and Ding, Shaojin and Xie, Jingyi and Yuan, Ye and Chen, Wuyang and Yang, Yang and Ren, Zhou and Wang, Zhangyang},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={8351--8361},
  year={2019}
}

@inproceedings{wei2018person,
  title={Person transfer gan to bridge domain gap for person re-identification},
  author={Wei, Longhui and Zhang, Shiliang and Gao, Wen and Tian, Qi},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={79--88},
  year={2018}
}

@inproceedings{zhong2019invariance,
  title={Invariance matters: Exemplar memory for domain adaptive person re-identification},
  author={Zhong, Zhun and Zheng, Liang and Luo, Zhiming and Li, Shaozi and Yang, Yi},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={598--607},
  year={2019}
}

@inproceedings{fu2019self,
  title={Self-similarity grouping: A simple unsupervised cross domain adaptation approach for person re-identification},
  author={Fu, Yang and Wei, Yunchao and Wang, Guanshuo and Zhou, Yuqian and Shi, Honghui and Huang, Thomas S},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={6112--6121},
  year={2019}
}

@inproceedings{zhai2020ad,
  title={Ad-cluster: Augmented discriminative clustering for domain adaptive person re-identification},
  author={Zhai, Yunpeng and Lu, Shijian and Ye, Qixiang and Shan, Xuebo and Chen, Jie and Ji, Rongrong and Tian, Yonghong},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={9021--9030},
  year={2020}
}

@inproceedings{ge2020mutual,
  title={Mutual Mean-Teaching: Pseudo Label Refinery for Unsupervised Domain Adaptation on Person Re-identification},
  author={Yixiao Ge and Dapeng Chen and Hongsheng Li},
  booktitle={International Conference on Learning Representations},
  year={2020},
  url={https://openreview.net/forum?id=rJlnOhVYPS}
}

@inproceedings{chendeep,
  title={Deep Credible Metric Learning for Unsupervised Domain Adaptation Person Re-identification},
  author={Chen, Guangyi and Lu, Yuhao and Lu, Jiwen and Zhou, Jie},
  booktitle={ECCV},
  year={2020}
}

@inproceedings{jin2020global,
  title={Global Distance-distributions Separation for Unsupervised Person Re-identification},
  author={Jin, Xin and Lan, Cuiling and Zeng, Wenjun and Chen, Zhibo},
  booktitle={ECCV},
  year={2020}
}

@misc{ge2020selfpaced,
        title={Self-paced Contrastive Learning with Hybrid Memory for Domain Adaptive Object Re-ID},
        author={Yixiao Ge and Dapeng Chen and Feng Zhu and Rui Zhao and Hongsheng Li},
        year={2020},
        eprint={2006.02713},
        archivePrefix={arXiv},
        primaryClass={cs.CV}
    }

@inproceedings{song2019generalizable,
  title={Generalizable person re-identification by domain-invariant mapping network},
  author={Song, Jifei and Yang, Yongxin and Song, Yi-Zhe and Xiang, Tao and Hospedales, Timothy M},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={719--728},
  year={2019}
}

@article{jia2019frustratingly,
  title={Frustratingly easy person re-identification: Generalizing person re-id in practice},
  author={Jia, Jieru and Ruan, Qiuqi and Hospedales, Timothy M},
  journal={arXiv preprint arXiv:1905.03422},
  year={2019}
}

@inproceedings{jin2020style,
  title={Style normalization and restitution for generalizable person re-identification},
  author={Jin, Xin and Lan, Cuiling and Zeng, Wenjun and Chen, Zhibo and Zhang, Li},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={3143--3152},
  year={2020}
}

@article{ulyanov2016instance,
  title={Instance normalization: The missing ingredient for fast stylization},
  author={Ulyanov, Dmitry and Vedaldi, Andrea and Lempitsky, Victor},
  journal={arXiv preprint arXiv:1607.08022},
  year={2016}
}

@inproceedings{tobin2017domain,
  title={Domain randomization for transferring deep neural networks from simulation to the real world},
  author={Tobin, Josh and Fong, Rachel and Ray, Alex and Schneider, Jonas and Zaremba, Wojciech and Abbeel, Pieter},
  booktitle={2017 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={23--30},
  year={2017},
  organization={IEEE}
}

@inproceedings{zhou2020learning,
  title={Learning to Generate Novel Domains for Domain Generalization},
  author={Zhou, Kaiyang and Yang, Yongxin and Hospedales, Timothy and Xiang, Tao},
  booktitle={ECCV},
  year={2020}
}

@inproceedings{li2018learning,
  title={Learning to generalize: Meta-learning for domain generalization},
  author={Li, D and Yang, Y and Song, Yi-Zhe and Hospedales, TM},
  booktitle={Proceedings of the Thirty-Second AAAI Conference on Artificial Intelligence (AAAI 2018)},
  pages={3490--3497},
  year={2018},
  organization={AAAI press}
}

@inproceedings{balaji2018metareg,
  title={Metareg: Towards domain generalization using meta-regularization},
  author={Balaji, Yogesh and Sankaranarayanan, Swami and Chellappa, Rama},
  booktitle={Advances in Neural Information Processing Systems},
  pages={998--1008},
  year={2018}
}

@inproceedings{dou2019domain,
  title={Domain generalization via model-agnostic learning of semantic features},
  author={Dou, Qi and de Castro, Daniel Coelho and Kamnitsas, Konstantinos and Glocker, Ben},
  booktitle={Advances in Neural Information Processing Systems},
  pages={6450--6461},
  year={2019}
}

@inproceedings{chen2017beyond,
  title={Beyond triplet loss: a deep quadruplet network for person re-identification},
  author={Chen, Weihua and Chen, Xiaotang and Zhang, Jianguo and Huang, Kaiqi},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={403--412},
  year={2017}
}

@article{hermans2017defense,
  title={In defense of the triplet loss for person re-identification},
  author={Hermans, Alexander and Beyer, Lucas and Leibe, Bastian},
  journal={arXiv preprint arXiv:1703.07737},
  year={2017}
}

@inproceedings{chen2019deep,
  title={Deep meta metric learning},
  author={Chen, Guangyi and Zhang, Tianren and Lu, Jiwen and Zhou, Jie},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={9547--9556},
  year={2019}
}

@inproceedings{sun2020circle,
  title={Circle loss: A unified perspective of pair similarity optimization},
  author={Sun, Yifan and Cheng, Changmao and Zhang, Yuhan and Zhang, Chi and Zheng, Liang and Wang, Zhongdao and Wei, Yichen},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={6398--6407},
  year={2020}
}

@inproceedings{zhao2017deeply,
  title={Deeply-learned part-aligned representations for person re-identification},
  author={Zhao, Liming and Li, Xi and Zhuang, Yueting and Wang, Jingdong},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={3219--3228},
  year={2017}
}

@inproceedings{li2017learning,
  title={Learning deep context-aware features over body and latent parts for person re-identification},
  author={Li, Dangwei and Chen, Xiaotang and Zhang, Zhang and Huang, Kaiqi},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={384--393},
  year={2017}
}

@inproceedings{suh2018part,
  title={Part-aligned bilinear representations for person re-identification},
  author={Suh, Yumin and Wang, Jingdong and Tang, Siyu and Mei, Tao and Mu Lee, Kyoung},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={402--419},
  year={2018}
}

@inproceedings{guo2019beyond,
  title={Beyond human parts: Dual part-aligned representations for person re-identification},
  author={Guo, Jianyuan and Yuan, Yuhui and Huang, Lang and Zhang, Chao and Yao, Jin-Ge and Han, Kai},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={3642--3651},
  year={2019}
}

@inproceedings{si2018dual,
  title={Dual attention matching network for context-aware feature sequence based person re-identification},
  author={Si, Jianlou and Zhang, Honggang and Li, Chun-Guang and Kuen, Jason and Kong, Xiangfei and Kot, Alex C and Wang, Gang},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={5363--5372},
  year={2018}
}

@inproceedings{song2018mask,
  title={Mask-guided contrastive attention model for person re-identification},
  author={Song, Chunfeng and Huang, Yan and Ouyang, Wanli and Wang, Liang},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={1179--1188},
  year={2018}
}

@inproceedings{chen2019mixed,
  title={Mixed high-order attention network for person re-identification},
  author={Chen, Binghui and Deng, Weihong and Hu, Jiani},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={371--381},
  year={2019}
}

@inproceedings{zhang2020relation,
  title={Relation-Aware Global Attention for Person Re-identification},
  author={Zhang, Zhizheng and Lan, Cuiling and Zeng, Wenjun and Jin, Xin and Chen, Zhibo},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={3186--3195},
  year={2020}
}

@inproceedings{chen2019self,
  title={Self-critical attention learning for person re-identification},
  author={Chen, Guangyi and Lin, Chunze and Ren, Liangliang and Lu, Jiwen and Zhou, Jie},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={9637--9646},
  year={2019}
}


@article{zhong2020learning,
  title={Learning to adapt invariance in memory for person re-identification},
  author={Zhong, Zhun and Zheng, Liang and Luo, Zhiming and Li, Shaozi and Yang, Yi},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2020},
  publisher={IEEE}
}

@article{song2020unsupervised,
  title={Unsupervised domain adaptive re-identification: Theory and practice},
  author={Song, Liangchen and Wang, Cheng and Zhang, Lefei and Du, Bo and Zhang, Qian and Huang, Chang and Wang, Xinggang},
  journal={Pattern Recognition},
  volume={102},
  pages={107173},
  year={2020},
  publisher={Elsevier}
}

@inproceedings{muandet2013domain,
  title={Domain generalization via invariant feature representation},
  author={Muandet, Krikamol and Balduzzi, David and Sch{\"o}lkopf, Bernhard},
  booktitle={International Conference on Machine Learning},
  pages={10--18},
  year={2013}
}

@inproceedings{ghifary2015domain,
  title={Domain generalization for object recognition with multi-task autoencoders},
  author={Ghifary, Muhammad and Bastiaan Kleijn, W and Zhang, Mengjie and Balduzzi, David},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={2551--2559},
  year={2015}
}

@inproceedings{li2018domain,
  title={Domain generalization with adversarial feature learning},
  author={Li, Haoliang and Jialin Pan, Sinno and Wang, Shiqi and Kot, Alex C},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={5400--5409},
  year={2018}
}

@inproceedings{carlucci2019domain,
  title={Domain generalization by solving jigsaw puzzles},
  author={Carlucci, Fabio M and D'Innocente, Antonio and Bucci, Silvia and Caputo, Barbara and Tommasi, Tatiana},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={2229--2238},
  year={2019}
}

@inproceedings{volpi2018generalizing,
  title={Generalizing to unseen domains via adversarial data augmentation},
  author={Volpi, Riccardo and Namkoong, Hongseok and Sener, Ozan and Duchi, John C and Murino, Vittorio and Savarese, Silvio},
  booktitle={Advances in neural information processing systems},
  pages={5334--5344},
  year={2018}
}

@inproceedings{shankar2018generalizing,
  title={Generalizing Across Domains via Cross-Gradient Training},
  author={Shankar, Shiv and Piratla, Vihari and Chakrabarti, Soumen and Chaudhuri, Siddhartha and Jyothi, Preethi and Sarawagi, Sunita},
  booktitle={International Conference on Learning Representations},
  year={2018}
}

@article{zhou2020domain,
  title={Domain Adaptive Ensemble Learning},
  author={Zhou, Kaiyang and Yang, Yongxin and Qiao, Yu and Xiang, Tao},
  journal={arXiv preprint arXiv:2003.07325},
  year={2020}
}

@inproceedings{li2019episodic,
  title={Episodic training for domain generalization},
  author={Li, Da and Zhang, Jianshu and Yang, Yongxin and Liu, Cong and Song, Yi-Zhe and Hospedales, Timothy M},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={1446--1455},
  year={2019}
}


@article{bilen2017universal,
  title={Universal representations: The missing link between faces, text, planktons, and cat breeds},
  author={Bilen, Hakan and Vedaldi, Andrea},
  journal={arXiv preprint arXiv:1701.07275},
  year={2017}
}

@inproceedings{rebuffi2018efficient,
  title={Efficient parametrization of multi-domain deep neural networks},
  author={Rebuffi, Sylvestre-Alvise and Bilen, Hakan and Vedaldi, Andrea},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={8119--8127},
  year={2018}
}

@inproceedings{dvornik2020selecting,
  title={Selecting Relevant Features from a Universal Representation for Few-shot Classification},
  author={Dvornik, Nikita and Schmid, Cordelia and Mairal, Julien},
  booktitle={ECCV},
  year={2020}
}

@article{liu2020universal,
  title={A Universal Representation Transformer Layer for Few-Shot Image Classification},
  author={Liu, Lu and Hamilton, William and Long, Guodong and Jiang, Jing and Larochelle, Hugo},
  journal={arXiv preprint arXiv:2006.11702},
  year={2020}
}

@inproceedings{rebuffi2018efficient,
  title={Efficient parametrization of multi-domain deep neural networks},
  author={Rebuffi, Sylvestre-Alvise and Bilen, Hakan and Vedaldi, Andrea},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={8119--8127},
  year={2018}
}

@article{luo2019strong,
  title={A strong baseline and batch normalization neck for deep person re-identification},
  author={Luo, Hao and Jiang, Wei and Gu, Youzhi and Liu, Fuxu and Liao, Xingyu and Lai, Shenqi and Gu, Jianyang},
  journal={IEEE Transactions on Multimedia},
  year={2019},
  publisher={IEEE}
}

@inproceedings{wen2016discriminative,
  title={A discriminative feature learning approach for deep face recognition},
  author={Wen, Yandong and Zhang, Kaipeng and Li, Zhifeng and Qiao, Yu},
  booktitle={European conference on computer vision},
  pages={499--515},
  year={2016},
  organization={Springer}
}

@inproceedings{zheng2015scalable,
  title={Scalable person re-identification: A benchmark},
  author={Zheng, Liang and Shen, Liyue and Tian, Lu and Wang, Shengjin and Wang, Jingdong and Tian, Qi},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={1116--1124},
  year={2015}
}

@inproceedings{zheng2017unlabeled,
  title={Unlabeled samples generated by gan improve the person re-identification baseline in vitro},
  author={Zheng, Zhedong and Zheng, Liang and Yang, Yi},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={3754--3762},
  year={2017}
}

@inproceedings{li2013locally,
  title={Locally aligned feature transforms across views},
  author={Li, Wei and Wang, Xiaogang},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={3594--3601},
  year={2013}
}

@inproceedings{li2014deepreid,
  title={Deepreid: Deep filter pairing neural network for person re-identification},
  author={Li, Wei and Zhao, Rui and Xiao, Tong and Wang, Xiaogang},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={152--159},
  year={2014}
}

@article{xiao2016end,
  title={End-to-end deep learning for person search},
  author={Xiao, Tong and Li, Shuang and Wang, Bochao and Lin, Liang and Wang, Xiaogang},
  journal={arXiv preprint arXiv:1604.01850},
  volume={2},
  number={2},
  year={2016}
}

@inproceedings{hirzer2011person,
  title={Person re-identification by descriptive and discriminative classification},
  author={Hirzer, Martin and Beleznai, Csaba and Roth, Peter M and Bischof, Horst},
  booktitle={Scandinavian conference on Image analysis},
  pages={91--102},
  year={2011},
  organization={Springer}
}

@article{loy2010time,
  title={Time-delayed correlation analysis for multi-camera activity understanding},
  author={Loy, Chen Change and Xiang, Tao and Gong, Shaogang},
  journal={International Journal of Computer Vision},
  volume={90},
  number={1},
  pages={106--129},
  year={2010},
  publisher={Springer}
}

@inproceedings{gray2008viewpoint,
  title={Viewpoint invariant pedestrian recognition with an ensemble of localized features},
  author={Gray, Douglas and Tao, Hai},
  booktitle={European conference on computer vision},
  pages={262--275},
  year={2008},
  organization={Springer}
}

@inproceedings{wei2009associating,
  title={Associating groups of people},
  author={Wei-Shi, Zheng and Shaogang, Gong and Tao, Xiang},
  booktitle={Proceedings of the British Machine Vision Conference},
  pages={23--1},
  year={2009}
}

@inproceedings{gray2007evaluating,
  title={Evaluating appearance models for recognition, reacquisition, and tracking},
  author={Gray, Douglas and Brennan, Shane and Tao, Hai},
  booktitle={Proc. IEEE international workshop on performance evaluation for tracking and surveillance (PETS)},
  volume={3},
  number={5},
  pages={1--7},
  year={2007},
  organization={Citeseer}
}

@article{zhang2017alignedreid,
  title={Alignedreid: Surpassing human-level performance in person re-identification},
  author={Zhang, Xuan and Luo, Hao and Fan, Xing and Xiang, Weilai and Sun, Yixiao and Xiao, Qiqi and Jiang, Wei and Zhang, Chi and Sun, Jian},
  journal={arXiv preprint arXiv:1711.08184},
  year={2017}
}

@article{nichol2018first,
  title={On first-order meta-learning algorithms},
  author={Nichol, Alex and Achiam, Joshua and Schulman, John},
  journal={arXiv preprint arXiv:1803.02999},
  year={2018}
}

@inproceedings{qiao2018few,
  title={Few-shot image recognition by predicting parameters from activations},
  author={Qiao, Siyuan and Liu, Chenxi and Shen, Wei and Yuille, Alan L},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={7229--7238},
  year={2018}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@article{opitz2018deep,
  title={Deep metric learning with bier: Boosting independent embeddings robustly},
  author={Opitz, Michael and Waltner, Georg and Possegger, Horst and Bischof, Horst},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  year={2018},
  publisher={IEEE}
}

@inproceedings{ye2020distilling,
  title={Distilling Cross-Task Knowledge via Relationship Matching},
  author={Ye, Han-Jia and Lu, Su and Zhan, De-Chuan},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={12396--12405},
  year={2020}
}

@inproceedings{rosenstein2005transfer,
  title={To transfer or not to transfer},
  author={Rosenstein, Michael T and Marx, Zvika and Kaelbling, Leslie Pack and Dietterich, Thomas G},
  booktitle={In NIPS’05 Workshop, Inductive Transfer: 10 Years Later},
  year={2005},
  organization={Citeseer}
}

@inproceedings{guo2018multi,
  title={Multi-Source Domain Adaptation with Mixture of Experts},
  author={Guo, Jiang and Shah, Darsh and Barzilay, Regina},
  booktitle={Proceedings of the 2018 Conference on Empirical Methods in Natural Language Processing},
  pages={4694--4703},
  year={2018}
}

@article{jacobs1991adaptive,
  title={Adaptive mixtures of local experts},
  author={Jacobs, Robert A and Jordan, Michael I and Nowlan, Steven J and Hinton, Geoffrey E},
  journal={Neural computation},
  volume={3},
  number={1},
  pages={79--87},
  year={1991},
  publisher={MIT Press}
}

@article{breiman2001random,
  title={Random forests},
  author={Breiman, Leo},
  journal={Machine learning},
  volume={45},
  number={1},
  pages={5--32},
  year={2001},
  publisher={Springer}
}

@article{amit1997shape,
  title={Shape quantization and recognition with randomized trees},
  author={Amit, Yali and Geman, Donald},
  journal={Neural computation},
  volume={9},
  number={7},
  pages={1545--1588},
  year={1997},
  publisher={MIT Press}
}

@inproceedings{paisitkriangkrai2015learning,
  title={Learning to rank in person re-identification with metric ensembles},
  author={Paisitkriangkrai, Sakrapee and Shen, Chunhua and Van Den Hengel, Anton},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={1846--1855},
  year={2015}
}

@inproceedings{cheng2016person,
  title={Person re-identification by multi-channel parts-based cnn with improved triplet loss function},
  author={Cheng, De and Gong, Yihong and Zhou, Sanping and Wang, Jinjun and Zheng, Nanning},
  booktitle={Proceedings of the iEEE conference on computer vision and pattern recognition},
  pages={1335--1344},
  year={2016}
}

@inproceedings{matsukawa2016hierarchical,
  title={Hierarchical gaussian descriptor for person re-identification},
  author={Matsukawa, Tetsu and Okabe, Takahiro and Suzuki, Einoshin and Sato, Yoichi},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1363--1372},
  year={2016}
}

@inproceedings{zhang2016learning,
  title={Learning a discriminative null space for person re-identification},
  author={Zhang, Li and Xiang, Tao and Gong, Shaogang},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1239--1248},
  year={2016}
}

@inproceedings{bai2017scalable,
  title={Scalable person re-identification on supervised smoothed manifold},
  author={Bai, Song and Bai, Xiang and Tian, Qi},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={2530--2539},
  year={2017}
}

@inproceedings{zhao2017spindle,
  title={Spindle net: Person re-identification with human body region guided feature decomposition and fusion},
  author={Zhao, Haiyu and Tian, Maoqing and Sun, Shuyang and Shao, Jing and Yan, Junjie and Yi, Shuai and Wang, Xiaogang and Tang, Xiaoou},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1077--1085},
  year={2017}
}

@inproceedings{bak2017one,
  title={One-shot metric learning for person re-identification},
  author={Bak, Slawomir and Carr, Peter},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={2990--2999},
  year={2017}
}

@inproceedings{su2016deep,
  title={Deep attributes driven multi-camera person re-identification},
  author={Su, Chi and Zhang, Shiliang and Xing, Junliang and Gao, Wen and Tian, Qi},
  booktitle={European conference on computer vision},
  pages={475--491},
  year={2016},
  organization={Springer}
}

@inproceedings{peng2016unsupervised,
  title={Unsupervised cross-dataset transfer learning for person re-identification},
  author={Peng, Peixi and Xiang, Tao and Wang, Yaowei and Pontil, Massimiliano and Gong, Shaogang and Huang, Tiejun and Tian, Yonghong},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1306--1315},
  year={2016}
}

@inproceedings{lin2018multi,
  title={Multi-task mid-level feature alignment network for unsupervised cross-dataset person re-identification},
  author={Lin, Shan and Li, Haoliang and Li, Chang Tsun and Kot, Alex Chichung},
  booktitle={29th British Machine Vision Conference, BMVC 2018},
  year={2018}
}

@inproceedings{wang2018transferable,
  title={Transferable joint attribute-identity deep learning for unsupervised person re-identification},
  author={Wang, Jingya and Zhu, Xiatian and Gong, Shaogang and Li, Wei},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={2275--2284},
  year={2018}
}

@inproceedings{bak2018domain,
  title={Domain adaptation through synthesis for unsupervised person re-identification},
  author={Bak, Slawomir and Carr, Peter and Lalonde, Jean-Francois},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={189--205},
  year={2018}
}

@article{he2020fastreid,
  title={Fastreid: A pytorch toolbox for general instance re-identification},
  author={He, Lingxiao and Liao, Xingyu and Liu, Wu and Liu, Xinchen and Cheng, Peng and Mei, Tao},
  journal={arXiv preprint arXiv:2006.02631},
  year={2020}
}

@inproceedings{finn2017model,
  title={Model-Agnostic Meta-Learning for Fast Adaptation of Deep Networks},
  author={Finn, Chelsea and Abbeel, Pieter and Levine, Sergey},
  booktitle={ICML},
  year={2017}
}

@article{fan2018unsupervised,
  title={Unsupervised person re-identification: Clustering and fine-tuning},
  author={Fan, Hehe and Zheng, Liang and Yan, Chenggang and Yang, Yi},
  journal={ACM Transactions on Multimedia Computing, Communications, and Applications (TOMM)},
  volume={14},
  number={4},
  pages={1--18},
  year={2018},
  publisher={ACM New York, NY, USA}
}

@inproceedings{deng2018image,
  title={Image-image domain adaptation with preserved self-similarity and domain-dissimilarity for person re-identification},
  author={Deng, Weijian and Zheng, Liang and Ye, Qixiang and Kang, Guoliang and Yang, Yi and Jiao, Jianbin},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={994--1003},
  year={2018}
}

@inproceedings{li2019cross,
  title={Cross-dataset person re-identification via unsupervised pose disentanglement and adaptation},
  author={Li, Yu-Jhe and Lin, Ci-Siang and Lin, Yan-Bo and Wang, Yu-Chiang Frank},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={7919--7929},
  year={2019}
}

@inproceedings{zhang2019self,
  title={Self-training with progressive augmentation for unsupervised cross-domain person re-identification},
  author={Zhang, Xinyu and Cao, Jiewei and Shen, Chunhua and You, Mingyu},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={8222--8231},
  year={2019}
}

@inproceedings{zhuang2020rethinking,
  title={Rethinking the Distribution Gap of Person Re-identification with Camera-Based Batch Normalization},
  author={Zhuang, Zijie and Wei, Longhui and Xie, Lingxi and Zhang, Tianyu and Zhang, Hengheng and Wu, Haozhe and Ai, Haizhou and Tian, Qi},
  booktitle={European Conference on Computer Vision},
  pages={140--157},
  year={2020},
  organization={Springer}
}

@inproceedings{d2018domain,
  title={Domain generalization with domain-specific aggregation modules},
  author={D’Innocente, Antonio and Caputo, Barbara},
  booktitle={German Conference on Pattern Recognition},
  pages={187--198},
  year={2018},
  organization={Springer}
}

@inproceedings{liu2020open,
  title={Open Compound Domain Adaptation},
  author={Liu, Ziwei and Miao, Zhongqi and Pan, Xingang and Zhan, Xiaohang and Lin, Dahua and Yu, Stella X and Gong, Boqing},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={12406--12415},
  year={2020}
}
